CriticAL: Critic Automation with Language Models

Understanding the world through models is a fundamental goal of scientific research. While large language model (LLM) based approaches show promise in automating scientific discovery, they often overlook the importance of criticizing scientific models. Criticizing models deepens scientific understanding and drives the development of more accurate models. Automating model criticism is difficult because it traditionally requires a human expert to define how to compare a model with data and evaluate if the discrepancies are significant--both rely heavily on understanding the modeling assumptions and domain. Although LLM-based critic approaches are appealing, they introduce new challenges: LLMs might hallucinate the critiques themselves. Motivated by this, we introduce CriticAL (Critic Automation with Language Models). CriticAL uses LLMs to generate summary statistics that capture discrepancies between model predictions and data, and applies hypothesis tests to evaluate their significance. We can view CriticAL as a verifier that validates models and their critiques by embedding them in a hypothesis testing framework. In experiments, we evaluate CriticAL across key quantitative and qualitative dimensions. In settings where we synthesize discrepancies between models and datasets, CriticAL reliably generates correct critiques without hallucinating incorrect ones. We show that both human and LLM judges consistently prefer CriticAL's critiques over alternative approaches in terms of transparency and actionability. Finally, we show that CriticAL's critiques enable an LLM scientist to improve upon human-designed models on real-world datasets.

==> alg_tex/report_discrepancy.tex <==
\begin{algorithm}[ht!]
\caption{Returning significant discrepancies} 
\label{alg:cap}
\KwIn{
dataset $\mathcal{Y}$,
probabilistic model $q$, 
number of proposals $m$}
\begin{algorithmic}[!ht]
\STATE Sample posterior predictive replicates $\{Y^{\text{rep}}_i\}_{i=1}^N \sim q(Y|\mathcal{Y})$ \\ 
\State Get $\{T_k\}_{k=1}^m$, $\{p_k \}_{k=1}^m$ from Algorithm~\ref{alg:proposal}. \\ 
\State $\{\tilde{p}_k\}_{k=1}^m  = \texttt{multiple-test-adjustment}(\{p_k\}_{k=1}^m)$
\label{alg:discrepancy}
\end{algorithmic}
\KwOut{
$T_k$ satisfying \(\tilde{p}_k \leq \alpha\)}
\end{algorithm}


==> figure_tex/experiment_1/ppc_comparison_exp1.tex <==
\begin{figure*}
\centering
\includegraphics[scale=0.60]{figures/experiment_1/ppc_experiment_1.pdf}
\caption{\textbf{Transforming CriticAL-proposed summary statistics into }
Test statistic distributions compared for (no discovery) Student's t/Student's t and Student's t/Gaussian (discovery). 
We plot the test statistic computed on the data as a vertical dashed line.
CriticAL proposes \texttt{kurtosis} which can distinguish between Gaussian and Student-t which the prespecified \texttt{mean} cannot.
}
\label{fig:exp:exp_1_test_stat_dist}
\end{figure*}

==> figure_tex/experiment_2/stan_criticism.tex <==
\begin{figure*}
\centering
\includegraphics[scale=0.525]{figures/experiment_2/discoveries.pdf}
\caption{\textbf{CriticAL discoveries for real-world model-dataset pairs.}
Percentage of model-dataset pairs flagged with at least one discrepancy against significance threshold. The pre-specified baseline does not identify any discrepancies except at high significance thresholds (likely to be false alarms).
}
\label{fig:exp:discoveries}
% \vspace{mm}
\end{figure*}

==> figure_tex/programs/mesquite_example.tex <==
\begin{figure*}[ht!]
\centering
\begin{tcolorbox}[
title={}]
\fontsize{7pt}{7pt}\selectfont
\ttfamily
\begin{lstlisting}[language=Python]
import numpy as np
from scipy.stats import skew
def test_statistic(df):
    # df['y_rep'] contains the posterior predictive sample of the leaf weight
    return = skew(df['y_rep'])
\end{lstlisting}

\begin{lstlisting}[language=Python]
def gen_model(observed_data):
    weight = np.log(observed_data['weight'].values)  # Log transformation of the response variable

    with pm.Model() as model:
        # Linear model
        mu = (beta[0] + beta[1]*diam1 + beta[2]*diam2 + beta[3]*canopy_height +
              beta[4]*total_height + beta[5]*density + beta[6]*group)        
        # Likelihood (sampling distribution) of observations
        y_obs = pm.StudentT("y_obs", mu=mu, sigma=sigma, nu=nu, observed=weight)
        
        # Sampling
        trace = pm.sample(5000, tune=1000, target_accept=0.90, chains=4, cores=1, random_seed=rng1, idata_kwargs={"log_likelihood": True})
        posterior_predictive = pm.sample_posterior_predictive(trace, random_seed=rng2, return_inferencedata=False)
        
        return model, posterior_predictive, trace

\end{lstlisting}

\end{tcolorbox}
\caption{\textbf{Test statistics drive modeling choices} \textbf{(top)}
\textbf{(bottom)} 
}
\label{code:test_statistic_informs_modeling}
\end{figure*}




==> figure_tex/programs/radon_pooled.tex <==
\begin{figure*}[ht!]
\centering
\begin{tcolorbox}[
title={}]
\fontsize{7pt}{7pt}\selectfont
\ttfamily
\begin{lstlisting}[language=Python]
def test_statistic(df):
    # The test statistic is the ratio of empirical variance in posterior predictive samples of log_radon
    # between basement and first floor measurements.

    # Filter rows pertaining to basement (coded, e.g., as 0) and first floor (coded as 1)
    basement_samples = df[df['floor_measure'] == 0]['y_rep']
    first_floor_samples = df[df['floor_measure'] == 1]['y_rep']

    # Calculate variances at each floor measure
    var_basement = np.var(basement_samples)
    var_first_floor = np.var(first_floor_samples)

    # Safety check to avoid division by zero
    if var_first_floor == 0:
        ratio_variances = None  # indicates a problem or degenerate scenario
    else:
        ratio_variances = var_basement / var_first_floor
\end{lstlisting}


\begin{lstlisting}[language=Python]

'''
Given the discrepancy identified in the previous model, which suggests that the model fails to capture the different variabilities of radon levels expected between different floor levels, we need to revise the model to account for these differences. The previous model used a single variance term for all observations, which is likely inappropriate given the data characteristics.

To address this, we can model the variance of the radon levels as dependent on the floor measurement. This approach will allow the model to have different variances for basement and first floor measurements, which should better capture the observed data structure.
'''
Here's the revised probabilistic program:

import pymc as pm
import numpy as np
import pandas as pd

def gen_model(observed_data):
    # Convert observed_data columns to numpy arrays
    floor_measure = observed_data['floor_measure'].values
    log_radon = observed_data['log_radon'].values
    log_uppm = observed_data['log_uppm'].values

    # Set seeds for reproducibility
    rng1 = np.random.default_rng(42)
    rng2 = np.random.default_rng(314)

    with pm.Model() as model:
        # Priors for intercept and slopes
        alpha = pm.Normal("alpha", mu=0, sigma=10)
        beta_floor = pm.Normal("beta_floor", mu=0, sigma=10)
        beta_uppm = pm.Normal("beta_uppm", mu=0, sigma=10)

        # Separate variance for basement and first floor
        sigma_basement = pm.HalfNormal("sigma_basement", sigma=1)
        sigma_first_floor = pm.HalfNormal("sigma_first_floor", sigma=1)
        
        # Model error based on floor measurement
        sigma_y = pm.math.switch(pm.math.eq(floor_measure, 0), sigma_basement, sigma_first_floor)

        # Expected value of outcome
        mu = pm.Deterministic("mu", alpha + beta_floor * floor_measure + beta_uppm * log_uppm)

        # Likelihood (sampling distribution) of observations
        y_obs = pm.Normal("y_obs", mu=mu, sigma=sigma_y, observed=log_radon)

        # Sampling
        trace = pm.sample(5000, tune=1000, target_accept=0.90, chains=4, cores=1, random_seed=rng1, idata_kwargs={"log_likelihood": True})
        posterior_predictive = pm.sample_posterior_predictive(trace, random_seed=rng2, return_inferencedata=False)

        return model, posterior_predictive, trace

\end{lstlisting}

\end{tcolorbox}
\caption{\textbf{Test statistics drive modeling choices} \textbf{(top)}
\textbf{(bottom)} 
}
\label{code:test_statistic_informs_modeling}
\end{figure*}




